So Different Yet So Alike! Constrained Unsupervised Text Style Transfer

Automatic transfer of text between domains has become popular in recent times. One of its aims is to preserve the semantic content of text being translated from source to target domain. However, it does not explicitly maintain other attributes between the source and translated text, for e.g., text length and descriptiveness. Maintaining constraints in transfer has several downstream applications, including data augmentation and de-biasing. We introduce a method for such constrained unsupervised text style transfer by introducing two complementary losses to the generative adversarial network (GAN) family of models. Unlike the competing losses used in GANs, we introduce cooperative losses where the discriminator and the generator cooperate and reduce the same loss. The first is a contrastive loss and the second is a classification loss, aiming to regularize the latent space further and bring similar sentences across domains closer together. We demonstrate that such training retains lexical, syntactic, and domain-specific constraints between domains for multiple benchmark datasets, including ones where more than one attribute change. We show that the complementary cooperative losses improve text quality, according to both automated and human evaluation measures.

==> Don't change that!/sections/acknowledgments.tex <==
\section*{Acknowledgments}

We would like to thank the anonymous reviewers for their useful suggestions.
We would also like to acknowledge the support of the NExT research grant funds, supported by the National Research Foundation, Prime Ministers Office, Singapore under its IRC@ SG Funding Initiative, and to gratefully acknowledge the support of NVIDIA Corporation with the donation of the GeForce GTX Titan XGPU used in this research. The work is also supported by the project no. T2MOE2008 titled CSK-NLP: Leveraging Commonsense Knowledge for NLP awarded by Singapore's Ministry of Education under its Tier-2 grant scheme.

==> Don't change that!/sections/conclusion.tex <==
\section{Conclusion}
Text style transfer works focuses on retaining content and changing the style of sentences but does not maintain other desirable constraints. We address this by introducing two cooperative losses to the GAN-inspired Adversarially Regularized Autoencoder (ARAE) that further regularizes the latent space. While satisfying the constraints 
% effectively, 
% irrespective of multiple attributes changing, 
our methods brings significant improvements in overall score.  While we focus on simple constraints at the sentence- and word-level, future work can add phrase-level and more fine-grained constraints.
% MinACL: I thought you already do this?
% the syntactic tree structure. 
Potential future work may explore reinforcement learning losses to directly optimize the constraints.

% and producing adversarial examples from different domains for a given NLP task. 
% MinACL: not very useful.  Omitting.
% We hope that the future style transfer works consider satisfying constraints while focusing on improving other metrics.

==> Don't change that!/sections/discussion.tex <==
\section{Discussion and Limitations}
\label{section:discussion}

% MinACL: you need an intro to this section.  How are these questions different than those in the previous subsections?

\paragraph{Cycle Consistency Loss:} a) \textit{In Latent Spaces} -
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Discussion on how cycle consistency in latent spaces don't work
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Cycle consistency in latent spaces has been shown to improve word-level tasks, such as cross-lingual dictionary construction \cite{mohiuddin-joty-2019-revisiting} and topic modeling \cite{hu-etal-2020-neural}. A recent work from \cite{huang-etal-2020-cycle} claims to improve unsupervised style transfer using such losses. In our experiments, however, it did not result in any noticeable performance improvement \footnote{Repeated attempts to obtain source codes failed.}. Given this, we hypothesize that cycle consistency might be too restrictive for sentence-level tasks. b) \textit{Using Back-Translation}- 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Discussion on how cycle consistency using Back-Translation is a costly affair and might not be needed. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Back-translation is another alternative to ensure semantic consistency between source and the target sentence \cite{prabhumoye-etal-2018-style, artetxe2018unsupervised, lample_unsupervised_mt}. 
% MinACL: your explanation here is a cop-out.  Why bother to raise it if you're not going to do it?  Wastes space.
However, in our case, since we are training an \arae{}, it would involve an additional inference and auto-encoder training step which is expensive and we defer exploring this. 

\paragraph{Using Transformers:} We also replace our LSTM auto-encoders with both pre-trained and randomly initialized 
% MinACL: if it was better, shouldn't you at least report lines in your tables for this system?
transformer encoder--decoders \cite{rothe-etal-2020-leveraging}. Although we found an increase in the \aggmetric{}, it was mostly because of very high \simmetric{} and very low \accmetric{}. 
Reducing the number of layers, attention heads would still result in a large model that is still prone to copying text. This reveals the potential limitations of our method and training using transformers is a  future work.

% -----
% MinACL: I thought you already went over applications in the introduction.  Why put it here (again)?  I'd omit it.

% \textbf{Applications of Constrained Style Transfer:} 
% We find several use cases of performing constrained style transfer. Apart from improving the intended task of style transfer --- which calls for achieving the change in style (or attribute) with minimal changes to the original text such that meaning is preserved --- our approach finds downstream applications that has practical significance. 

% MinACL: BUG empty section.
% \textbf{Use in Stylistic Rewriting and Copy Editing}:

% MinACL: perhaps show such sentences in place of Fig. 1? So that your 
\paragraph{Transferred sentences as Adversarial Examples:}
We demonstrate an important application of our proposed constrained transfer by considering them as adversarial examples for domain adaptation. Domain Adversarial Neural Network (DANN) \cite{DBLP:series/acvpr/GaninUAGLLML17} is an unsupervised domain adaptation method that improves performance of an end-task (e.g, sentiment analysis) on a target domain considering only supervised data from source domain. We train DANN for sentiment analysis on amazon reviews dataset \cite{mcauleydataset} with {\sc DVD} as source and {\sc Electronics} as the target domain -- achieving an accuracy of 83.75\% on {\sc electronics}. 

Next, we train the best variant of \systemname{} to transfer a separate set {\sc DVD} reviews to {\sc Electronics} reviews and use them as adversarial examples to test the DANN model \footnote{Since each of {\sc DVD} and {\sc electronics} contain positive and negative reviews, we test whether transferred sentences maintain the appropriate sentiment and find the accuracy to be 79\%.}. We find that the accuracy of DANN on the {\sc electronics} domain reduces by $\sim$3 points. This shows the potential application of domain transferred sentences as adversarial examples. Similar ideas have been tried for image style transfer \cite{DBLP:journals/corr/abs-2004-12385}, but needs more investigation in NLP.  


% We use reviews from the {\sc DVD} and {\sc Electronics} domain where every domain contains both positive and negative reviews. We first train a Domain Adversarial Neural Network (DANN) \cite{DBLP:series/acvpr/GaninUAGLLML17} --- a unsupervised domain adaptation method that considers labeled data from {\sc DVD} and unlabeled data from {\sc Electronics} --- achieving an accuracy of 83.75\% on electronics domain. Separately, we also train our best model to transfer {\sc DVD} reviews to {\sc Electronics} reviews. We find that the transferred sentences maintain the sentiment of the reviews 79\% of the time as a sanity check. Further, we use the transferred sentences 
% % MinACL: Syntax error --- missing verb.
% to domain adversarial neural networks and find that the accuracy of DANN reduced by $\sim$3 points. 


==> Don't change that!/sections/experiments.tex <==
\section{Experiments}
\begin{table}[t!]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{|l l c c c c c|}
        \hline
        \textbf{Dataset} & \textbf{Attributes} & \textbf{Train} & \textbf{Dev} & \textbf{Test} & \makecell{\textbf{Avg} \\\textbf{len.}} & \textbf{Vocab}   \\
        \hline
        \multirow{2}{4em}{\yelpdata}  & Positive & 266,041 & 25,278 & 50,278 & \multirow{2}{1em}{8.9}  & \multirow{2}{1em}{10K} \\
         & Negative & 177,218 & 38,205 & 76,392 &  &\\
        \hline
        \multirow{2}{4em}{\imdbdata}  & Positive & 178,869 & 2K & 1K & 
         \multirow{2}{1em}{18.5} & \multirow{2}{1em}{30K} \\
         & Negative & 187,597 & 2K & 1K & & \\
        \hline
        \multirow{2}{4em}{\politicaldata}  & Democratic & 270,000 & 2K & 28K & \multirow{2}{1em}{16} & \multirow{2}{1em}{30K} \\
         & Republican  & 270,000 & 2K & 28K & & \\
        \hline
    \end{tabular}
    }
    \caption{Dataset splits for \yelpdata, \imdbdata~and \politicaldata. }
    \label{tab:dataset-splits}
\end{table}

\begin{table*}[t!]
    \centering
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{|l|l| c c c c | c c c c| c c c c|}
         \hline
          && \multicolumn{4}{c}{\textbf{\yelpdata{}}} & \multicolumn{4}{c}{\textbf{\imdbdata{}}} & \multicolumn{4}{c|}{\textbf{\politicaldata{}}} \\
         \textbf{Model}&\textbf{Sampling} & \textbf{\textsc{acc}} & \textbf{\textsc{fl}} & \textbf{\textsc{sim}} & \textbf{\aggmetric{}} & \textbf{\textsc{acc}} & \textbf{\textsc{fl}} & \textbf{\textsc{sim}} & \textbf{\aggmetric{}} & \textbf{\textsc{acc}} & \textbf{\textsc{fl}} & \textbf{\textsc{sim}} & \aggmetric{} \\
         
         \toprule[0.5pt]  
        
        %  \multicolumn{13}{c}{{\bf \textsc{drg and arae (in that order)}}}  \\
         \hline
         \textbf{\textsc{drg}}&greedy & 67.4 & 54.5 & \textbf{43.6} & 16.7 & 56.5 & 44.3 & \textbf{54.1} & 14.4 & 61.3 & 35.7 & 38.7 & 8.8 \\ 
         
        \textbf{\textsc{arae}}& greedy & \textbf{93.1} & 67.9 & 31.2 & 19.8 & 95.0 & 76.3 & 26.4 & 19.9 & 63.0 & 72.1 & 17.3 & 11.0 \\
         
         \hline
        %  \multicolumn{13}{c}{{\bf \systemname{}}} \\
         \hline
         \multirow{2}{*}{\bf \systemname{}} & greedy  & 88.3 & 66.0 & 34.4 & 20.2 & 95.4 &	70.5 &	\textbf{36.4} &	26.0  & 95.80	& 53.1	& 28.5 & 	14.1  \\ 
         
         & nucleus($p=0.6$) & 86.7 & 63.9 & 35.3 & 19.9 &  95.1 &	69.8 &	\textbf{36.4} &	25.6  & 95.8	& 52.2 & 	28.4 & 	13.9   \\ 
         
        %  &0.9 & 88.3	& 64.1	& 33.8	& 19.5  &  95.3	 & 66.3 & 	35.9	& 24.0 & 95.80	 & 50.5	 & 28.0	 & 13.2  \\ 
         
         \hline
        %  \multicolumn{13}{c}{{\bf \systemname{} + \textsc{clf}}} \\
         \hline

         
         \multirow{2}{*}{\makecell[l]{\bf \systemname{} \\ \hspace{0.5cm} +  \bf \textsc{clf}}} &greedy & 85.7	 & 63.4	 & 36.7 & 20.2 &  96.0 & 73.6	& 35.4	& 26.2  & 98.6	& 55.0	& \textbf{44.4}	& \textbf{25.5} \\ 
         
         & nucleus($p=0.6$) & 85.6 & 63.0 & 36.6 & 20.0 & 95.8	& 72.8	& 35.3	& 25.7  & 98.6 &	54.4 &	44.2 &	25.1 \\ 
         
        %  &0.9 & 85.8 &	61.8 &	36.1 &	19.5 & 95.8	& 71.1	& 34.7	& 25.0   & 98.6	& 52.6	& 43.4	& 24.1    \\ 
         
         
         \hline
        %  \multicolumn{13}{c}{{\bf \systemname{} + \textsc{contra}}} \\
         \hline
         
         \multirow{2}{*}{\makecell[l]{\bf \systemname{} \\ \hspace{0.5cm} +  \bf \textsc{contra}}}  & greedy & 89.6	& \textbf{69.7} & 32.0	& 20.1 & 97.6 &	82.9 &	32.5 &	27.0  & 99.0	& 56.5	& 40.8	& 24.2 \\ 
         
         & nucleus($p=0.6$) & 89.7	 & 69.2	 & 31.9 & 	20.0  & 97.7 & 83.2 & 32.2	& 26.7   &  99.0 & 55.9 &	40.7 &	23.9  \\ 
         
        %  &0.9 & 89.7	 & 67.7 &	31.5 &	19.3  & 97.4 & 81.4 & 	32.0	& 25.9  & 99.0 & 54.3 & 39.9 &	22.8  \\ 
         
         \hline
        %  \multicolumn{13}{c}{{\bf \systemname{} + \textsc{clf} + \textsc{contra}}} \\
         \hline
         % MinACL: can you break these system names across multiple names so that the first column is less wide?  Then you can bump up the font size.
         \multirow{2}{*}{\makecell[l]{\bf \systemname{} \\ \hspace{0.5cm} +  \bf \textsc{clf}  + \textsc{contra}}} &greedy & 89.3 & 69.2  &  32.9 &  \textbf{20.6} & \textbf{97.8}	& \textbf{84.0} & 33.5 &	\textbf{28.1}  & \textbf{99.0}	& \textbf{56.8}	& 41.8	& 24.9  \\ 
         
         & nucleus($p=0.6$)& 89.4 & 68.6 & 32.8 & 20.4  & 97.1 & 82.6 & 33.6 & 27.4 & 99.0	& 56.0 & 41.6	& 24.4  \\ 
         
        %  &0.9 & 89.5 & 67.0 & 32.3 & 19.7 & 97.8	& 82.0	& 33.1	& 27.2  &  99.0	& 54.6	& 40.8	& 23.5 \\ 

         
         \hline
    \end{tabular}
    }
    % MinACL: you don't say why the figures are bold?
    \caption{Evaluation of \systemname{}~with \textsc{acc} (transfer accuracy), \textsc{fl} (fluency)  and \textsc{sim} (semantic similarity), \aggmetric{} (aggregate metric). Cooperatively reducing the contrastive or the classification loss is better than \arae{}. We report the mean of five runs for our experiments. The bolded measures are the best results}
    \label{tab:main-results}
\end{table*}

\paragraph{Datasets.} We use three datasets with single attribute changes:
$i)$~\textbf{Yelp Reviews}:  business reviews listed on Yelp, labeled as either a positive or negative sentiment. $ii)$~\textbf{IMDb Movie Reviews}: 
consists of movie reviews \cite{dai-etal-2019-style} also labelled as positive or negative. $iii)$~\textbf{Political Slant}: consists of Facebook posts from the politicians of the United States Senate and the House of Representatives \cite{prabhumoye-etal-2018-style}, labeled with either democratic/republican slant. 
% See \Cref{sec:dataset-statistics} for dataset statistics.

We provide a summary of the dataset statistics in \Cref{tab:dataset-splits}. We include datasets of varied length and complexity. Apart from having different topics,  the \imdbdata \ dataset is more formal compared to the more colloquial \yelpdata. We fix the maximum vocabulary size for \yelpdata{}, \imdbdata{} and \politicaldata{} at 30K which is also the default maximum vocab size used in \cite{DBLP:conf/icml/ZhaoKZRL18}.




\paragraph{Constraints:}
We constrain every sentence along \textit{six} diverse dimensions that we desire to control between the two domains: 
% MinACL: how is length a lexical constraint?
$i)$~\textbf{Lexical}: \textit{Sentence length} -- The transferred sentence should maintain a length similar to the original sentence (binarized to long sentences with 10 or or more words or short otherwise). $ii)$~\textbf{Syntactic}:
Presence of personal pronouns (binarized to indicate the presence of a \textit{personal pronoun}); number of adjectives (categorical up to 5); number of proper nouns (categorical up to 3); syntactic tree height (categorical up to 10). 
% MinACL: likely need to give examples of what these are.  
$iii)$~\textbf{Domain specific} -- number of \textit{domain-specific attributes} \cite{li-etal-2018-delete} (categorical up to 5). 
% MinACL: what does this mean?
Further, we label the sentence with a constraint-specific, catch-all label if the bounds are beyond what we mention above. 
% MinACL: not clear what F1 on a constraint means.  Do you mean whether the constraint was broken or not?  If so, who judges?
Since the distribution of the labels may be different, we report the F1 score on our constraints.

\subsection{Model Details}
For the encoders, we use a one-layer LSTM network with 300 hidden dimensions for all the datasets. For the critics and classification loss, we use a two-layer multi-layer perceptron with 100 hidden units. 

% Our learning rates and methods to stabilize training are discussed in \Cref{sec:more-training-details}.

\noindent
\paragraph{Training Hyper-parameters:}
For all our experiments we set the learning rate of the auto-encoder ($lr_{ae}$) to 1e-3 and ($lr_{disc}$) to 1e-4. The number of discriminator steps ($n_{dis}$) is set to 5. The Adam optimizer parameters $\beta_1$=$0.5$ and $\beta_2$=$0.9$, which ensures a more conservative optimization and is known to improve stability. We also add a gradient penalty to the loss function of the discriminator that stabilizes training. All the suggestions for stabilizing training are mostly obtained from \cite{DBLP:conf/iclr/ArjovskyB17}.

\paragraph{Inference Hyper-parameters:}
We used nucleus sampling with $p \in [0.6, 0.9]$. We tried different temperatures of scaling the softmax \cite{DBLP:conf/icml/GuoPSW17} - 0.4, 0.5, 0.6, 0.7 and chose the one that produced the best result on the dev set.

\subsection{Evaluation Setup}

\paragraph{Automatic Evaluation:} Our automatic evaluation considers the following three prominent criteria: $i)$~\textbf{Semantic Similarity (\textsc{sim}):} Measured between source and translated target sentences using encoders \cite{wieting-etal-2019-beyond}, instead of \textit{n-gram} metrics like \textsc{bleu} \cite{papineni-etal-2002-bleu} which have weak correlations with human judgments. $ii)$~\textbf{Transfer Accuracy (\textsc{acc}):}  The transferred sentence should belong to the target domain and a classifier is trained to distinguish between the source and the target sentence. We use \textit{fastText} classifiers \cite{joulin2017bag} for every dataset. We achieve accuracy of $97.9$ for \yelpdata,\ $96.9$ for \imdbdata \ and $97.1$ for \politicaldata. $iii)$~\textbf{Fluency (\textsc{fl}):} A transferred sentence should be grammatically correct. We fine-tune a RoBERTa-large model on the COLA \cite{warstadt2018neural} dataset to indicate whether a sentence is linguistically acceptable. Finally, we combine the three scores into an aggregate, following the criteria suggested by \citet{krishna-etal-2020-reformulating}:
\begin{equation*}
    AGG = \frac{1}{|S|}\sum_{s \in S} \textit{\textsc{ACC} (s)} \cdot \textit{\textsc{SIM} (s)} \cdot \textit{\textsc{FL} (s)} 
\end{equation*}

\paragraph{Human Evaluation:} We also perform an indicative human evaluation where we randomly sample 100 samples from each of the three datasets and hire three researchers to rate every sentence for \flmetric{}, \simmetric{} and \accmetric{} on a 3-point scale \cite{krishna-etal-2020-reformulating}. 
% MinACL: who are these researchers?  Are they not you? If so, disclose.  Did you compensate your annotators?  Need to disclose that these are only indicative results.  Fixed for you in first sentence.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/numbers.pdf}
  \caption{F-scores of different constraints. Adding cooperative losses helps in better maintaining the constraints. The error bars show the variance of generating text using greedy decoding and nucleus sampling with $p=\{0.6,0.9\}$.}
  \label{fig:maintaining-constraints}
\end{figure*}

% \begin{figure*}[t]
%   \centering
%   \subfloat[Length]{
%   \includegraphics[scale=0.3]{figures/length.pdf}
%   }
%   \subfloat[Personal Pronouns]{
%   \includegraphics[scale=0.3]{figures/personal_df.pdf}
%   }
%   \subfloat[Proper Noun]{
%   \includegraphics[scale=0.3]{figures/prop_noun_df.pdf}
%   }\\
%   \subfloat[Descriptive]{
%   \includegraphics[scale=0.3]{figures/descriptive_df.pdf}
%   }
%   \subfloat[Tree Height]{
%   \includegraphics[scale=0.3]{figures/tree_height_df.pdf}
%   }
%   \subfloat[\# Domain Attributes]{
%   \includegraphics[scale=0.3]{figures/num_dom_attributes_df.pdf}
%   }
%   \caption{F-scores of different constraints from systems. Length, Personal Pronouns, Proper Nouns, Descriptiveness, Tree Height and Number of Domain specific attributes. Adding cooperative losses helps in better maintaining the constraints between two domains. The error bars show the variance of generating text using greedy decoding and nucleus sampling with $p=\{0.6,0.9\}$}
%   \label{fig:maintaining-constraints}
% \end{figure*}

% Details about the baseline.
% What does the baseline do 
% Are they state of the art?
\subsection{Baselines}
\label{sec:baselines-description}
We compare \systemname{} with the following baselines: \textbf{a) \textsc{drg}}: The Delete, Retrieve, Generate method that deletes domain specific attributes, retrieves a template and generates the target domain text \cite{li-etal-2018-delete}. We use the stronger, entire system rather than the weaker \textsc{deleteonly} and \textsc{retrieveonly} baselines; \textbf{b) \textsc{arae}}: Adversarially regularized autoencoders our system is based on \cite{DBLP:conf/icml/ZhaoKZRL18};
\textbf{c) \systemname{}}: Our model without the contrastive learning or cooperative classifier; \textbf{d) \systemname{} + \textsc{contra}}: Our model with the contrastive learning; \textbf{e) \systemname{} + \textsc{clf}}: Our  model with the cooperative classifier; \textbf{f) \systemname{}+\textsc{clf+contra}}: Our model with both the cooperative losses.
The closest model to ours is from \cite{huang-etal-2020-cycle}. However, we were not able to reproduce the results.\footnote{Repeated attempts to obtain the original source code failed.}



\subsection{Results}

\subsubsection{Overall Results}
\label{sec:overall-results}
% \begin{itemize} 
%     \item When contrastive learning is added, the main observation is that 
%     \flmetric{} consistently improves across datasets. 
%     \item \drg{} has good \textsc{sim} scores because most of the text is copied from the source sentence, but does not have good \textsc{acc}, as also noted by many other works.
%     \item{} \politicaldata{} has comparitively lower results because of larger vocabulary size.
% \end{itemize}
\systemname{} + \textsc{contra} and \systemname{} + \textsc{clf} consistently perform better than \drg{} and \arae{} on the \aggmetric{} score (\Cref{tab:main-results}). The \aggmetric{} for \yelpdata{} is 20.6 (vs. 19.8), for \imdbdata{} it is 28.1 (vs. 19.9) and for \politicaldata{} 25.5 (vs. 11.0). Although cooperative loss reduction aims to satisfy the constraints between two domains, our results show that further regularization of the latent space not only brings advantages in satisfying the constraints but also improves performance~\cite{integrating-categorical-semantics-GAN}.

% \noindent 
\textbf{Effect of Cooperative Loss Reduction on \accmetric{} \flmetric{} and \simmetric{}: } Across datasets, reducing cooperative losses improves  \accmetric{} and \flmetric{} and \simmetric{} to \arae{}. Although \drg{} produces sentences with high \simmetric{} as most of the text from the original sentence is retained after the delete step, there is a large trade-off with \accmetric{} resulting in low \aggmetric{} scores. Also, compared to \arae{}, adding cooperative losses significantly increases the \simmetric{}, with the highest increase observed for \politicaldata{}.
% MinACL: ok explanation but doesn't actually have much to do with the paper's topics it seems.
\abhi{The reasons for this could be two-fold: $i)$ since we mine positive sentences from a corpus that is grounded in real world events, most lexically-similar sentences may also be semantically similar}~\cite{guu-etal-2018-generating}, and $ii)$ since we tie the encoders from the source and target domain, we extract domain-agnostic information before generation, which retains content.

Fluency (\flmetric{}) also improves over all datasets. We hypothesize that reducing cooperative losses regularizes the latent space bringing fluent sentences closer together, enabling the decoder to produce semantically similar and linguistically acceptable sentences. The improvement for \politicaldata{} is less; we find these source sentences themselves are less fluent and contain many U.S. political acronyms, and that our system produces many out-of-vocabulary words affecting fluency.

% \noindent 
\textbf{Nucleus Sampling:} Our system achieves the highest \aggmetric{} score with greedy decoding. We also experiment with nucleus sampling \cite{nucleus-sampling} with different $p$ values. We report results for only $p$=$0.6$  in \Cref{tab:main-results}, as it produced the best result. With $p$=0.6, the results are  more diverse, increasing \accmetric{} as expected. However we find that with higher values of $p$, there is a trade-off with \simmetric{} resulting in a lower \aggmetric{} score overall --- similar to \citet{krishna-etal-2020-reformulating}.

% \noindent
\textbf{Effect of the Number of Positives:} The number of positive and negative samples used for contrastive learning (Eq. \ref{eq:contra-loss}) have a significant effect on the overall performance \cite{DBLP:conf/nips/KhoslaTWSTIMLK20, DBLP:conf/icml/ChenK0H20, pmlr-v119-henaff20a}. \Cref{tab:ablation-study} (\textit{rows} $|P|\in \{1,2,5,10\}$) shows the \aggmetric{} scores on  \imdbdata{} (for one of the runs), for different number of positives. We find that \aggmetric{} is the highest with 2 positives per sample as also used by \citet{DBLP:conf/nips/KhoslaTWSTIMLK20}. Although increasing the number of negatives is beneficial for contrastive learning, when more than one positive example is available, using them brings further improvements \cite{DBLP:conf/nips/KhoslaTWSTIMLK20}.

% \begin{table}[t!]
%     \small 
%     \centering
%     \begin{tabular}{|c|c|}
%     \hline
%     \# Positives ($P$) & \aggmetric \\
%     \hline
%     1 & 26.2 \\ 
%     2 & \textbf{28.6} \\ 
%     5 & 26.0 \\ 
%     10 & 26.0 \\ 
%     \hline
%     \end{tabular}
%     \caption{Effect of the number of positives used in contrastive learning on the \aggmetric{} metric for the \imdbdata{}}
%     \label{tab:effect-of-number-of-positives}
% \end{table}


% \noindent
\textbf{Cooperative Losses are Important on Both the Generator and Critic:}  \Cref{tab:ablation-study} shows the importance of adding the cooperative losses on the generator and critic. First, we see that adding the cooperative losses on both the generator and the critic is crucial for the overall performance. While adding the cooperative contrastive loss to both the generator and critic increases \flmetric{} and \accmetric{} while maintaining similar levels of \simmetric{}, adding the cooperative classification loss improves \simmetric{} which shows the complementary nature of the losses.  

\begin{table}[t!]
    \small 
    \centering
    \begin{tabular}{|c| c c c c|}
    \hline 
    \textbf{Model} & \textbf{\accmetric} & \textbf{\flmetric} & \textbf{\simmetric} &   \textbf{\aggmetric} \\
    \hline
    \hline
    \systemname{} + \textsc{clf} & 95.0 & 83.2 & 34.2 & 27.5 \\ 
    --~generator  & 96.2 & 87.2 & 31.3 & 26.7 \\ 
    --~critic & 94.9  & 84.4 & 30.8 & 25.5 \\
    \hline
    \hline
    \systemname{} + \textsc{contra} & 96.1 & 80.6 & 36 & 28.6 \\ 
    --~generator & 93.5 & 78.8 & 34.0 & 26.0 \\ 
    --~critic & 90.1 & 67.8  & 39.5 & 24.9 \\ 
    \hline
    \hline
    $|P|=1$ & 92.4 & 75.5 & 36.6 & 26.2  \\ 
    $|P|=2$  & 96.1 & 80.6 & 36.0 & 28.6  \\ 
    $|P|=5$  & 96.0  & 84.0  & 31.4 & 26.0  \\ 
    $|P|=10$  & 95.5 & 83.3 & 31.8 & 26.0  \\ 
    \hline 
    \end{tabular}
    \caption{Ablation study showing for cooperative losses not added to the generator (--generator) and the critic (--critic) and with different \# of positives on \imdbdata{}.}
    \label{tab:ablation-study}
\end{table}

% \noindent
\textbf{Human Evaluation:} We average the results and present it in \Cref{tab:human_eval}. \drg{} produces marginally better semantically similar sentences. Compared to \arae{}, our model performs well except for in \yelpdata{}. This may be because we use nucleus sampling with 0.9 which optimizes for diversity rather than similarity. On other metrics we perform on par or better than our competing systems. (See \Cref{sec:more-details-human-evaluation})


\begin{table}[t!]
    \small 
    \centering
    \begin{tabular}{|c| c| c c c|}
    \hline
    \textbf{Dataset} & \textbf{Model} & \textbf{\accmetric{}} & \textbf{\flmetric{}} & \textbf{\simmetric{}} \\
    \hline
    \multirow{3}{*}{\yelpdata{}} & \drg{}  &  2.3 &  2.1 & 2.1  \\
     &  \arae{} & \textbf{2.8} &  \textbf{2.4} &  \textbf{2.1} \\
     &  \textsc{ours} & \textbf{2.8}  & \textbf{2.4}  & 2.0  \\
    \hline
    \multirow{3}{*}{\imdbdata{}} & \drg{}  & 1.9  & 2.0  & \textbf{2.2}  \\
     &  \arae{} & 2.5  & 2.1 & 1.4 \\
     &  \textsc{ours} & \textbf{2.6}  & \textbf{2.2}  & 2.1  \\
    \hline 
    \multirow{3}{*}{\politicaldata{}} & \drg{}  & 2.3 & 2.2 & 2.1  \\
     &  \arae{} & 2.1 & 2.1 & 1.5  \\
     &  \textsc{ours} & \textbf{2.5}  & \textbf{2.4} & \textbf{2.2}  \\
    \hline
    \end{tabular}
% MinACL: we have no idea what the scores are.  BUG.  Is higher better?
\caption{Human evaluation of generated sentences.}
    \label{tab:human_eval}
\end{table}

\begin{table*}[]
    \centering
    \renewcommand\cellalign{lc}
    \setcellgapes{3pt}\makegapedcells
    \resizebox{\linewidth}{!}{
        \begin{tabular}{|l|l|l|l|}
        \hline
        \textbf{Dataset} & \textbf{Input} & \textbf{Output (Ours)} & \textbf{Output (\arae{})}  \\
        \hline
        \yelpdata{} & they close earlier than posted hours & they're open late night & they keep me getting better  \\
        \hline
        % \yelpdata{} & i will not go back to this hotel again & i will definitely go back again and again & i will definitely go back to return and again \\ 
        % \hline
        \imdbdata{} & \makecell[l]{this movie is a very poor attempt to \\ make money using a classical theme.} & \makecell[l]{this movie is a very good example \\ of a film that will never be forgotten.} & \makecell[l]{this is a film that has been a lot of times \\ and it's really good.} \\
        \hline
        % \imdbdata{} & \makecell[l]{it was wooden, totally unrealistic \\ and had no plot or meaning to the story} & \makecell[l]{it was also very funny, \\ and i was pleasantly surprised by the story} & \makecell[l]{it was also a great cast , and the \\ characters are so hard to find.} \\ 
        % \hline
        % \politicaldata{} & what are you doing about the border ? & what are what you are doing about gun violence? & so why are you and the republican party ? \\ 
        % \hline
        \politicaldata{} & i wish u would bring change  & and i wish you would help bring democracy & and i 'm not sure mr.trump.  \\
        \hline
        \end{tabular}
    }
    \caption{Example outputs generated by the best system according to \aggmetric{} score.}
    \label{tab:geneartions}
\end{table*}

% \noindent
% MinACL: insufficient narration for this section.  Should walk through examples and show how the below three problems are diagnosed.
\textbf{Qualitative Examples:}  \Cref{tab:geneartions} shows examples of the quality of transferred examples (see \Cref{sec:more-transfer-results} for more). 
Mistakes made by the model can be attributed to poor understanding of the original semantics, lack of diversity, and 
% MinACL: isn't this a big no-no?  I thought we want to guarantee attribute-specific words?
not producing attribute-specific words.

% General observation: Compared to other baselines, the cooperative loss reduction maintains the constraint in a better manner  
% Which constraints are harder to maintain and why?
% Why is there a spike in the IMDB proper noun results ? - An example. Proper nouns in the imdb data are mostly actor names or movie character names. These have very low tf.idf. So they are not deleted during generation and almost gets carried over to the target sentence 
% john forsythe was so bad and unfunny that he was actually annoying and irritating
% john forsythe gets retained in the content
% translated sentence: john c. scott and his show is actually a very funny and actually deserved .
% \\ overall, \textcolor{darkgreen}{i} was pleasantly surprised, this was one of the best animated films $\Vert$ \\ although this was n't one, it was nice, the first hour of an episode. }& \makecell[l]{Our model reproduces the word \textcolor{darkgreen}{"i"} \\even in the target sentence while ARAE misses it.}  \\ 

\begin{table}[t]
    \centering
    \renewcommand\cellalign{lc}
    \setcellgapes{3pt}\makegapedcells
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|l|l|}
    \hline 
    \textbf{Constraint} & &  \\
    \hline 
    \multirow{4}{*}{\makecell[l]{\textbf{Personal} \\ \textbf{Pronoun}}} & \makecell[l]{\textit{Source} (\imdbdata)} &\makecell[l]{jean seberg had not one iota of acting talent.} \\ 
    
    & \textit{Ours} &\makecell[l]{michael keaton was also great in his role.}\\
    
    & \textit{\arae{}} &\makecell[l]{john abraham had one of \colorbox{darkorange}{my} favorite roles .}\\
    
    % \hline
    
    % \multirow{3}{*}{\makecell[l]{\textbf{Personal} \\ \textbf{Pronoun}}} & \textit{Source Sentence (\imdbdata)} &\makecell[l]{oh ,\colorbox{darkgreen}{i} forgot,there was one redeeming feature - the scenery was nice} & 
    % \multirow{3}{*}{\makecell[l]{Our model reproduces the word \colorbox{darkgreen}{\textbf{i}} \\even in the target sentence while \arae{} misses it.}} \\
    
    % & \textit{Ours} & \makecell[l]{overall, \colorbox{darkgreen}{i} was pleasantly surprised, this was one of the best animated films}&\\
    
    % & \textit{\arae{}} &\makecell[l]{although this was n't one, it was nice, the first hour of an episode.}&\\
    
    \hline 
    
    \multirow{6}{*}{\makecell[l]{\textbf{Proper} \\ \textbf{Noun}}} & \makecell[l]{\textit{Source} (\imdbdata)} &\makecell[l]{\colorbox{Green1}{chris klein's} character was unlikable from \\  the start and never made an improvement} \\
    
    & \textit{Ours} & \makecell[l]{\colorbox{Green1}{robert de niro} was very good as the man \\ and she's never been}\\
    
    & \textit{\arae{}} &\makecell[l]{both of his character was made and \\ had a huge smile on me}\\

    \hline
    \end{tabular}
    }
    % MinACL: but the bottom example looks syntactically wrong and has poor semantics...  Can you find a better example?
    \caption{Table showing constraints satisfied by our system compared to \arae{}. Our method maintains constraints like number of proper nouns between sentences.}
    \label{tab:constraints-example}
\end{table}


\subsubsection{Maintaining Constraints}
\label{sec:results-maintaining-constraints}
\Cref{fig:maintaining-constraints} shows that introducing the cooperative losses significantly outperform \drg{} and \arae{} in maintaining constraints. Specifically  the \systemname{} + \textsc{clf} model performs better than \systemname + \textsc{contra}. One reason could be that, finding the appropriate positives and strong negatives can be problematic for contrastive learning. On the other hand, the classifier's objective is simpler and forces the encoder to produce representations that satisfy the different constraints effectively. 

A seemingly easy to maintain constraint is the length of the sentence. However,\ \textit{seq2seq} systems have a difficulty of maintaining appropriate lengths  \cite{murray-chiang-2018-correcting}. With no additional regularization \arae{} does not maintain the length as well as \systemname{} + \textsc{clf}. On the other hand, compared to the lexical constraints, syntactic attributes like descriptiveness, tree height and domain specific constraints present challenges, with significantly lower F scores. \systemname{} + \textsc{clf} produces significantly better results in maintaining them. This shows that obtaining improvements on the overall \aggmetric{} does not necessarily translate to producing outputs that satisfy constraints.
\drg{} maintains the proper noun for \imdbdata{} effectively, because it contains a wide variety of actor and movie names. They are retained verbatim after the delete operation. 

% For example, consider this sentence from the test dataset \textit{``John Forsythe was so bad and unfunny that he was actually annoying and irritating''}. The name \textit{``John Forsythe''} is a rare entity and remains after the delete operation. The translated sentence produced is \textit{John c. Scott and his show is actually a very funny and actually deserved .} Although the model hallucinates, it still produces a proper noun which explains why \drg{} effectively maintains most of the pronouns.

% Two datasets that can contain multiple attributes 
% \noindent
\textbf{Multiple Attribute Datasets:}
To test whether our model can satisfy constraints across domains where multiple attributes change, we use the multi-attribute dataset released by \cite{DBLP:conf/iclr/LampleSSDRB19}. We chose the {\sc Asian} and {\sc Mexican} as two domains. Each of these domains can have multiple attributes like positive and negative sentiment text, different gender attributions to sentences, etc. We compare our \systemname{} + \textsc{clf} model with the \systemname{} and \arae{} in \Cref{fig:multi-attribute-comparison}.  The results are more pronounced in this case with \systemname{} + \textsc{clf} having clear advantage over \systemname{}. This shows that even with multiple attributes changing between domains, cooperatively reducing losses can satisfy different constraints more effectively. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/multiattribute_constraints.pdf}
    \caption{Comparison of \arae{}, \systemname{} and \systemname{} + \textsc{clf} for different constraints.}
    \label{fig:multi-attribute-comparison}
\end{figure}



\textbf{Qualitative Examples:} 
\Cref{tab:constraints-example} shows examples of our model maintaining constraints compared to \arae{}.  Sometimes, \arae{} hallucinates and adds personal pronouns like ``my'' to the text even when there are no personal pronouns (\textit{row} 1). Also, our model produces sentences where the number of proper nouns are retained (Chris Klein vs. Robert De Niro), whereas \arae{} does not.



==> Don't change that!/sections/introduction.tex <==
\section{Introduction}

% % General Background 
% Humans are capable of mapping given inputs from one 
% % Min: this is not a domain.  Sounds more like application area or modality.
% % Abhi: Some ICLR papers do accept that even languages are different domains. I hope it is accepted in the NLP community.
% domain to the other. For example, machine translation converts text between languages, \cite{DBLP:conf/nips/VaswaniSPUJGKP17,artetxe2018unsupervised,lample_unsupervised_mt}, or emoji creation maps human faces to emojis \cite{DBLP:conf/iclr/TaigmanPW17}. Humans do these tasks efficiently, robustly, and without direct supervision. 
% % Specific Background 
% Recently, there has been a surge of interest in similar tasks such as attribute transfer \cite{jin2020deep} and controlled text generation  \cite{plug-play-language-model,multiple-attribute-text-style-transfer}.  These works aim to preserve the semantics of the source sentence (``content''), while changing certain attributes (``style''). Some common works include changing the sentiment \cite{li-etal-2018-delete}, expertise  \cite{cao-etal-2020-expertise}, formality \cite{formality-style-rao}, or multiple attributes \cite{multiple-attribute-text-style-transfer}. 

% The translation on the left does not have similar length, no personal noun and no domain specific proper noun compared to the higher fidelity translation on the right.  Domain transfer maintains constraints between the source and the target sentence unlike text style transfer.


Modern neural networks methods are capable of mapping data from one domain to another. Prominent examples include translation of text between languages~\cite{DBLP:conf/nips/VaswaniSPUJGKP17,artetxe2018unsupervised,lample_unsupervised_mt}, emoji creation from human faces \cite{DBLP:conf/iclr/TaigmanPW17}, and stylistic transfer of speech~\cite{yuan2021improving}. In Natural Language Processing (NLP),  the umbrella term \textit{attribute transfer}~\cite{jin2020deep} (or \textit{domain transfer}) refers to similar methods\footnote{While the literature primary utilizes the term \textit{style transfer}, we adopt the more general term \textit{attribute} as suggested by \citet{dijin-survey}.}. The aim is to maximally preserve the semantics of the source sentence (``content'') but change other properties (``attributes''), such as sentiment \cite{jin2020deep}, expertise \cite{cao-etal-2020-expertise}, formality  \cite{formality-style-rao} or a combination of them \cite{multiple-attribute-text-style-transfer}.

% Problems or the knowledge gap 
% While most relevant works, offered under the umbrella term \textit{text style transfer}, aim to preserve a vague definition of ``content'', they do not explicitly enforce any constraints of identity between the source and the translated text. For example, there is no explicit guarantee that the source and the transferred sentence will have a similar length or remain descriptive. \Cref{fig:illustrative_example} shows one such example, where a sentence from the books domain is translated to the movie domain. While the translated sentence ``Loved the Movie'' is an accepted text style transferred sentence because it retains much of the content and has the target attribute, it does not have the same length, does not have a personal noun (``I'') and does not have a domain appropriate proper noun. Comparatively, the higher-fidelity transfer ``I absolutely enjoyed Spielberg's direction '',  maintains constraints of identity and has the personal pronoun, along with a domain-appropriate proper noun. 

\textit{Text style transfer}, a popular form of attribute transfer, regards ``style'' as any attribute that changes between datasets \cite{dijin-survey}. Building on the progress of supervised transfer models, recent works have focused on \textit{unsupervised style transfer} that avoids costly annotation of parallel sentences. 
However, models built using unsupervised methods perform poorly when compared to supervised (parallel) training \cite{artetxe-etal-2020-call}. These methods, while capable of achieving the target domain characteristics, often fail to maintain the invariant content. \Cref{fig:illustrative_example} illustrates one such example, where a sentence from the 
% MinACL: TODO added sc formatting for domains.  Hope that it's ok and can be carried throughout.
{\sc Books} domain is translated to the {\sc Movie} domain. While the translated sentence ``\textit{Loved the movie}'' has correctly transferred the attribute (style), it does not have the same length, does not retain the personal noun (``\textit{I}''), nor use a domain-appropriate proper noun. Comparatively, the higher-fidelity transfer ``\textit{I absolutely enjoyed Spielberg's direction}'', maintains such \textit{constraints of identity}, in addition to being apt.

% \begin{table}[t!]
%     \centering
%     \begin{tabular}{@{}l@{}}
%     \toprule
%     \colorbox{darkorange}{\bf \textsc{\textcolor{white}{camera}}}: I bought the camera for my 8 year old to learn about digital photography. \\ 
%     \colorbox{darkblue}{\bf \textsc{\textcolor{white}{book}}}: I bought the book for my kid to learn how to read. \\ 
%     \colorbox{darkblue}{\bf \textsc{\textcolor{white}{book}}}: I bought the book for my second kid to teach him to read. \\
%     \colorbox{darkgreen}{\bf \textsc{\textcolor{white}{Kitchen}}}: I bought the oven for my 8 year old to learn baking \\ 
%     \colorbox{darkgreen}{\bf \textsc{\textcolor{white}{Kitchen}}}: I got a juicer for my partner, for him to stay healthy. \\ 
%     \colorbox{violet}{\bf \textsc{\textcolor{white}{Electronics}}}: I purchased a xbox for my partner to entertain himself. \\ 
%     \hline 
%     \colorbox{darkblue}{\bf \textsc{\textcolor{white}{book}}}: I am a huge John Grishman fan. \\
%     \colorbox{darkorange}{\bf \textsc{\textcolor{white}{camera}}}: I am a Canon fan. \\ 
%     \colorbox{darkgreen}{\bf \textsc{\textcolor{white}{Kitchen}}}: I only have Samsung appliances in my kitchen. \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{Examples showing cross domain generation. The top row shows the source domain sentence (From the Amazon Reviews Dataset). The subsequent rows show similar text in another domain. Note: The examples are generated by Abhinav and not by any NLP system.}
%     \label{tab:domain-transfer-main-exs}
% \end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/illustrative_example.pdf}
    \caption{\footnotesize Illustrative example showing transfer of text from books to movies while maintaining constraints of identity. 
    }
    \label{fig:illustrative_example}
\end{figure}


% In this work, we are concerned with a more general topic of Cross-domain generation, which is different from style transfer as the variant (and invariant) attributes between two domains might not be explicitly known. This arises due to the fact that the definition of domains and the corresponding differences in attributes between two arbitrary domains might not be known apriori (cite barbara plank).  \cite{DBLP:conf/iclr/TaigmanPW17} solve similar domain transfer for images where the only constraint for the transfer is that perceptual function $f$ produces similar representations on examples from the two domains. They argue that domain transfer models can solve style transfer but not vice-versa.

% MinACL: moving this paragraph from the final part of the introduction to earlier 
This problem setting is an important application of text transfer, as 
enforcing constraints of identity can help maintain the brand identity when the product descriptions are mapped from one commercial product to another. They can also help in data augmentation for downstream domain adaptation NLP applications (\cref{section:discussion}). Constraints of identity are explored extensively in the computer vision task of cross-domain image generation.
% MinACL: I have a hard time seeing the relevance of this below related work. I'd drop it.
% AbhiACL: I have changed it
\cite{DBLP:conf/iclr/TaigmanPW17}, but these issues---to the best of our knowledge---are  unexplored in NLP.


In this paper, we improve unsupervised attribute transfer by enforcing invariances via explicit constraints. 
Current methods in text attribute transfer lack mechanisms to explicitly enforce such constraints between the source and the transferred sentence. To this end, we build upon unsupervised text style transfer work by introducing an additional explicit regularization component in the latent space of a GAN-based \textit{seq2seq} network through two complementary losses (\cref{sec:method}). Unlike the adversarial losses in the GAN framework, our proposed losses cooperatively reduce the same objective. The first loss is a contrastive loss \cite{contrastive_learning_review} that brings sentences that have similar constraints closer and pushes sentences that are dissimilar farther away. The second loss is a classification loss that helps maintain the sentence identity via constraints from the latent vectors \cite{acgan}.

Our approach, while simple and aimed at maintaining constraints, improves the overall performance of the generation. We demonstrate these gains over three datasets: \yelpdata{} \cite{DBLP:conf/icml/ZhaoKZRL18}, \imdbdata{} \cite{dai-etal-2019-style} and \politicaldata{} \cite{prabhumoye-etal-2018-style}, generating six constraints including lexical, syntactic and domain-specific constraints. The introduced cooperative losses satisfy the constraints more effectively compared against strong baselines. Since multiple attributes can change between two domains \cite{multiple-attribute-text-style-transfer}, we test our method on one such dataset and show that the constraints of identity are maintained more effectively (\Cref{sec:results-maintaining-constraints}). 
% MinACL: This paragraph isn't necessary I think.  Restructured.  I also changed NLP => NLG.
% In summary our contributions are: 
% 1) 
To the best of our knowledge, our approach is the first to introduce cooperative losses in a GAN-like setup for NLG. 
% MinACL: removed 2, since it doesn't add value.
% 2) Maintain constraints of identity for text style transfer while improving overall quality.

% \begin{itemize}[leftmargin=*]
%     \itemsep-2pt
%     \item We identify that maintaining constraints of identity is necessary for text style transfer and introduce two losses that are cooperatively reduced by the generators and critic of \arae{} -- a combination which to the best of our knowledge has not been explored in NLP. 
%     % Although, it is aimed to maintain constraints of identity between two domains, it improves the over all performance compared to strong baselines.
%     \item We show that the introduced cooperative losses regularize the latent space effectively and help in maintaining the constraints in a better manner, while also improving the over all quality. 
% \end{itemize}

==> Don't change that!/sections/method.tex <==
\section{Preliminaries}

\paragraph{Task Setup:} We consider two sets of sentences (or corpora) \srcdom{}$=\{x_{src}^1, x_{src}^2, \dots x_{src}^{m}\}$ and \trgdom{}$=\{x_{trg}^1, x_{trg}^2, \dots x_{trg}^{n}\}$, as the \textit{source} and \textit{target} domains, respectively. Each corpus --- which we interpret as domains --- contain discernable attributes, ranging from sentiment (e.g., positive vs. negative), topics, political slant (e.g., democratic vs. republican), or some combination \cite{li-etal-2018-delete,DBLP:conf/iclr/LampleSSDRB19}. The overall task is to rewrite a piece of text $s_i \in \text{\srcdom{}}$ to $t_i \in \text{\trgdom{}}$, such that the translation changes the attributes varying across the two domains but retains the remaining content. While content retention is not explicitly defined in the literature, we design this new task of constrained unsupervised attribute transfer that assigns explicit constraints $\mathcal{C} = \{c_1, c_2, \ldots, c_{|\mathcal{C}|}\}$, to be retained. These constraints can be defined at various levels of a sentence: lexical, syntactic and domain-specific.

\begin{figure*}[t!]
    \centering
    \subfloat[ \label{fig:vanilla-dct}]{\includegraphics[width=0.45\textwidth]{figures/model/vanilla-dct.pdf}} 
    \hspace{0.8cm}
    \subfloat[\label{fig:contra-clf-dct}]{\includegraphics[width=0.45\textwidth]{figures/model/contrastive_arae.pdf}} 
    \caption{(a) \systemname{} -- We replace the generator of \arae{} with an encoder that encodes text from $\mathcal{T}$. (b) Adding our proposed cooperative losses to the model.}
    \label{fig:architecture}
\end{figure*}

\paragraph{Adversarially Regularized Autoencoder} (\arae{}): To perform unsupervised attribute transfer, we consider \textit{seq2seq} models that encode source sentences to a latent space and then decodes them to the target sentences. \arae{}s \cite{DBLP:conf/icml/ZhaoKZRL18} are the auto-encoder variants of the Generative Adversarial Network (GAN) \cite{DBLP:journals/corr/GoodfellowPMXWOCB14} framework. They learn smooth latent spaces (by imposing implicit priors) to ease the sampling of latent sentences. \arae{}s have been widely adopted in tasks like unsupervised text generation \cite{huang-etal-2020-cycle}, topic modeling \cite{hu-etal-2020-neural}, among others, and form the backbone of our proposed model.

\arae{} consists of an auto-encoder with a deterministic encoder $\displaystyle enc_{\theta}: \mathcal{X} \rightarrow \mathcal{Z}$ that encodes sentences into a latent space; i.e., $\mathbf{z} = enc_{\theta}(\mathbf{x}) \sim P_{z}$, and a conditional decoder $p_\phi(\mathbf{x}|\mathbf{z})$ that generates a sentence given a latent code. \arae{} regularizes this latent space utilizing a GAN-like setup that includes an implicit prior obtained from a parameterized generator network $enc_{\psi}: \mathcal{N}(0,I) \rightarrow \mathcal{Z}$. Here,  $enc_{\psi}$ maps a noise sample $s \sim \mathcal{N}(0,I)$ to the corresponding prior latent code $\mathbf{\bar{z}} = enc_{\psi}(s) \sim P_{\bar{z}}$.

A critic $\displaystyle crc_{\xi}: \mathcal{Z}  \rightarrow \mathbb{R}$ then learns to distinguish between real and generated samples, whereas both $enc_{\theta}$ and  $enc_{\psi}$ are adversarially trained to fool the critic. This results in a minimax optimization which implicitly minimizes the JS-Divergence between the two distributions $\displaystyle P_{z}$ and $\displaystyle P_{\bar{z}}$:

% MinCR too much vspace.  Try to shrink.
\begin{equation}
    \underset{\psi}{\min} \ \underset{\xi}{\max}  \quad 
    \underset{\mathbf{z} \sim P_{z}}{\mathbb{E}}[crc_{\xi}(\mathbf{z})] - \underset{\mathbf{\bar{z}} \sim P_{\bar{z}}}{\mathbb{E}}[crc_{\xi}(\mathbf{\bar{z}})] \label{Eq:original-minimax}
\end{equation}

% The min-max optimization requires careful balancing of the different loss functions and makes the training unstable. A common technique used to improve the stability of GANs is to replace the discriminator $\displaystyle D_{\xi}$ with a critic $\displaystyle C_{\xi}: \mathcal{Z} \times \tilde{\mathcal{Z}} \rightarrow \mathbb{R}.$, that produces greater values for real samples and smaller values for fake samples. Instead of the implicit JS-Divergence, this reduces the Wasserstein distance between $\displaystyle P_{\tilde{z}}$ and $\displaystyle P_{z}$. \cite{pmlr-v70-arjovsky17a}
The training involves three optimizations: $i)$ reducing the auto-encoder loss $\mathcal{L}_{ae}$, which tries to reconstruct the input and encourages copying behavior and maintain semantics similar to the original text (Eq.~\ref{Eq:autoencoder-training}); $ii)$ optimizing the critic's loss $\mathcal{L}_{cri}$ to distinguish between real and fake samples (Eq.~\ref{Eq:disc-training}) $iii)$ training the encoder and generator $\mathcal{L}_{adv}$ to fool the critic (Eq.~\ref{Eq:adv-training}):

\begin{eqnarray}
    \mathcal{L}_{ae}(\theta, \phi)=\underset{\mathbf{z} \sim P_{z}}{\mathbb{E}}[-\log\ p_{\phi}(\mathbf{x} | \mathbf{z})]  \label{Eq:autoencoder-training} \\
    \mathcal{L}_{crc}(\xi)=\underset{\mathbf{z} \sim P_{z}}{-\mathbb{E}}[ crc_{\xi}(\mathbf{z}) ] + \underset{\mathbf{\bar{z}} \sim P_{\bar{z}}}{\mathbb{E}} [crc_{\xi}(\mathbf{\bar{z}}) ]  \label{Eq:disc-training} \\
    \mathcal{L}_{adv}(\theta, \psi)=\underset{\mathbf{z} \sim P_{z}}{\mathbb{E}}[crc_{\xi}(\mathbf{z}) ] - \underset{\mathbf{\bar{z}} \sim P_{\bar{z}}}{\mathbb{E}}[crc_{\xi}(\mathbf{\bar{z}}) ] \label{Eq:adv-training} 
\end{eqnarray}

\section{Proposed Method} \label{sec:method}

\subsection{Base Model (\systemname{})} While \arae{} is an auto-encoder that recreates input $\mathbf{x} \rightarrow \mathbf{\hat{x}}$, our requirement is to translate sentences from one domain to another. Given this, we modify the \arae{} to a \textit{seq2seq} variant such that we can translate input sentences between source and target domains; i.e., $\mathbf{x}_{src} \rightarrow \mathbf{\hat{x}}_{tgt}$ and $\mathbf{x}_{tgt} \rightarrow \mathbf{\hat{x}}_{src}$.

To achieve this, we  utilize $enc_\theta$ to encode $\mathbf{x}_{src}$ and repurpose $enc_\psi$ to encode $\mathbf{x}_{tgt}$. We obtain their latent codes $(\mathbf{z},\mathbf{\bar{z}})$ which we name as $(\mathbf{z}^s,\mathbf{z}^t)$, i.e., $\mathbf{z}^s = enc_\theta(\mathbf{x}_{src})$ and $\mathbf{z}^t = enc_\psi(\mathbf{x}_{tgt})$.

Next, to generate sentences, we consider two decoders $\mathbf{\hat{x}}_{src} \sim p_\phi(\mathbf{x}|\mathbf{z})$ and $\mathbf{\hat{x}}_{tgt} \sim p_\eta(\mathbf{x}|\mathbf{z})$. Here, $\mathbf{z}$ can be either $\mathbf{z}^s$ or $\mathbf{z}^t$ based on whether we auto-encode (e.g., $p_\phi\left(\mathbf{x}|\mathbf{z}^s=enc_\theta(\mathbf{x}_{src})\right)$) or translate (e.g., $p_\phi\left(\mathbf{x}|\mathbf{z}^t=enc_\psi(\mathbf{x}_{tgt})\right)$). Unlike \arae{}'s single decoder, we incorporate two decoders to enable bi-directional translation.

In the above process, instead of sampling $s$ from a noise distribution like $\mathcal{N}(0, I)$ and passing it through a generator $enc_{\psi}$, we feed it text from the target domain \trgdom{} and a decoder $dec_{\eta}$ that decodes text in \trgdom{}. This is inspired from Cycle-GAN \cite{DBLP:conf/iccv/ZhuPIE17}, where instead of matching the noise distribution $\mathcal{N}$, we match the distribution of \trgdom{}.
% MinACL: Is there a good reason why you do this above point instead?  Seems like it needs some explanation.
% AbhiACL: Changed this a little bit.

In addition, we tie the weights of the encoders from both domains, so that the encoders learn to encode domain-agnostic information. Tying encoder weights has also been used by unsupervised machine translation \cite{artetxe2018unsupervised,lample_unsupervised_mt}
and multiple other works \cite{DBLP:conf/emnlp/MaiPMSH20, huang-etal-2020-cycle,hu-etal-2020-neural, artetxe2018unsupervised}\footnote{We tried with separate encoders and decoders, but encoders with tied weights work best}. 

\begin{algorithm}[t!]

 \For{each training iteration} {
    \colorbox{Gray2}{1) Train the Auto-encoders:} \\ 
       {\Indp Sample $\; \mathbf{x}_{src} \sim \mathcal{S} \;$,
        $\; \mathbf{x}_{trg} \sim \mathcal{T}$ \\ 
        $\mathbf{z}^s = enc_{\theta}(\mathbf{x}_{src}),\ \mathbf{z}^t = enc_{\psi}(\mathbf{x}_{trg})$ \\ 
        Backprop loss, $\mathcal{L}_{ae}(\theta, \phi)$, $\mathcal{L}_{ae}(\psi, \eta)$\\}
        
    \colorbox{Green2}{2) Train the Critic:} \\
        
        {\Indp Sample $\; \mathbf{x}_{src} \sim \mathcal{S} \;$,
        $\; \mathbf{x}_{trg} \sim \mathcal{T}$ \\ 
        $\mathbf{z}^s = enc_{\theta}(\mathbf{x}_{src}),\ \mathbf{z}^t = enc_{\psi}(\mathbf{x}_{trg})$ \\
        $\mathbf{z}_{crc}^s = crc_{\xi}^{hid}(\mathbf{z}^s),~\mathbf{z}_{crc}^t = crc_{\xi}^{hid}(\mathbf{z}^t)$ \\ 
    
        $l_{crc} \leftarrow \mathcal{L}_{crc}(\xi)$ \\ }
        
    \colorbox{Green1}{2a) Critic Co-op Training:} \\ 
        
        {\Indp 
        Backprop loss, $l_{crc} + \lambda_1\mathcal{L}_{con}(\xi) + \lambda_2\mathcal{L}_{clf}(\xi,~\delta)$ \\
        }
    
    \colorbox{Blue2}{3) Adversarial Training:} \\
        {\Indp 
        Sample $\; \mathbf{x}_{src} \sim \mathcal{S} \;$,
        $\; \mathbf{x}_{trg} \sim \mathcal{T}$ \\ 
        $\mathbf{z}^s = enc_{\theta}(\mathbf{x}_{src}),\ \mathbf{z}^t = enc_{\psi}(\mathbf{x}_{trg})$ \\ 
        Backprop loss, $\mathcal{L}_{adv}(\theta, \psi)$\\ 
        }
        
    \colorbox{Blue1}{3a) Encoder Co-op Training:} \\ 
        {\Indp 
        Backprop loss, $\lambda_1\mathcal{L}_{con}(\theta,~\phi) + \lambda_2\mathcal{L}_{clf}(\theta,~\phi,~\delta)$ \\
        }
 }
\caption{\systemname{} + \textsc{clf} + \textsc{contra}}
\label{algo:training-algo}
\end{algorithm}


% \begin{algorithm}[t!]
% \small
% \SetAlgoLined
% \SetKwInOut{Input}{Input}


% \Input{
% \# iteration of critic\ / iteration of enc: $n_{dis}$, lrs- autoencoder: $lr_{ae}$, critic: $lr_{dis}$, adv train: $lr_{adv}$. Adam params: $\beta_1, \beta_2$.
% }
%  Initialize $(\theta, \phi, \psi, \eta, \xi, \delta)$ \\ 
%  \For{1, \dots \# iterations} {
%     \textit{\textbf{(1) Train the autoencoders}} \\ 
%         $\mathbf{x_{src}} \leftarrow \{x_{src}^i\}_{i=1}^{m}\sim\mathcal{S}$ \\ 
%         $\mathbf{x_{trg}} \leftarrow \{x_{trg}^j\}_{j=1}^{n}\sim\mathcal{T}$ \\ 
%         $\mathbf{z^s} = enc_{\theta}(\mathbf{x_{src}}),\ \mathbf{z^t} = enc_{\psi}(\mathbf{x_{trg}})$ \\ 
%         $\theta,~\phi \leftarrow$ Adam($\mathcal{L}_{ae}(\mathbf{z^s}; \theta, \phi),~\beta_1,~\beta_2,~lr_{ae})$ \\
%         $\psi,~\eta \leftarrow$ Adam(${\mathcal{L}_{ae}(\mathbf{z^t}; \psi, \eta),~\beta_1,~\beta_2,~lr_{ae}}$) \\
%     \textit{\textbf{(2) Train the Critic}} \\
%     \For{1, \dots \# $n_{dis}$} {
%         $\mathbf{x_{src}} \leftarrow \{x_{src}^i\}_{i=1}^{m}\sim\mathcal{S}$ \\ 
%         $\mathbf{x_{trg}} \leftarrow \{x_{trg}^j\}_{j=1}^{n}\sim\mathcal{T}$ \\ 
%         $\mathbf{z^s} = enc_{\theta}(\mathbf{x_{src}}),\ \mathbf{z^t} = enc_{\psi}(\mathbf{x_{trg}})$ \\ 
%         \tcp{Last layer representations} 
%         $\mathbf{z_{cri}^s} = C_{\xi}^{hid}(\mathbf{z^s}),~\mathbf{z_{cri}^t} = C_{\xi}^{hid}(\mathbf{z^t})$   \\ 
%         $l_{cri} \leftarrow \mathcal{L}_{cri}(\mathbf{z^s},~\mathbf{z^t};~\xi)$ \\ 
%         \textcolor{algohighlight}{\textit{\textbf{(2a) Critic Cooperative Training}}} \\ 
%         \textcolor{algohighlight}{$l_{cri}^{con} \leftarrow \mathcal{L}_{con}(\mathbf{z_{cri}^s},~\mathcal{C};~ \xi)$} \ \tcp*{contrastive loss} 
%         \textcolor{algohighlight}{$l_{cri}^{clf} \leftarrow \mathcal{L}_{clf}([\mathbf{z_{cri}^s}; \mathbf{z_{cri}^t}],~\mathcal{C}_{i};~\xi,~\delta$)} \ \tcp*{clf loss} 
%         $\mathcal{L}_{cri} \leftarrow l_{cri} + \textcolor{algohighlight}{\lambda_1 l_{cri}^{con}} + \textcolor{algohighlight}{\lambda_2l_{cri}^{clf}}$ \\
%         $\xi \leftarrow$ Adam($\mathcal{L}_{cri},~\beta_1,~\beta_2,~lr_{dis}$) \\
%     }
%     \textit{\textbf{(3) Adversarial Training}} \\
%     \textit{\textbf{(3a) Adv Training of Target Encoder}} \\
%     $\mathbf{x_{trg}} \leftarrow \{x_{trg}^j\}_{j=1}^{n}\sim\mathcal{T}$ \\ 
%     $\mathbf{z^t} = enc_{\theta}(\mathbf{x_{trg}})$ \\ 
%     $\theta \leftarrow Adam(\underset{\mathbf{z^t}}{\mathbb{E}}[C_{\xi}(\mathbf{z^t})],~\beta_1,~\beta_2,~lr_{adv})$ \\
%     \textit{\textbf{(3b) Adv Training of Source Encoder}} \\
%     $\mathbf{x_{src}} \leftarrow \{x_{src}^i\}_{i=1}^{m}\sim\mathcal{S}$ \\ 
%     $\mathbf{z^s} = enc_{\theta}(\mathbf{x_{src}})$ \\
%     $\psi \leftarrow Adam(-\underset{\mathbf{z^s}}{\mathbb{E}}[C_{\xi}(\mathbf{z_t})],~\beta_1,~\beta_2,~lr_{adv})$ \\
%     \textcolor{algohighlight}{\textit{\textbf{(4) Encoder Cooperative Training}}} \\ 
%     $\mathbf{x_{src}} \leftarrow \{x_{src}^i\}_{i=1}^{m}\sim\mathcal{S}$ \\ 
%     $\mathbf{x_{trg}} \leftarrow \{x_{trg}^j\}_{j=1}^{n}\sim\mathcal{T}$ \\ 
%     $\mathbf{z^s} = enc_{\theta}(\mathbf{x_{src}}),\ \mathbf{z^t} = enc_{\psi}(\mathbf{x_{trg}})$ \\ 
%     \textcolor{algohighlight}{$l_{enc}^{con} \leftarrow \mathcal{L}_{con}(\mathbf{z^s},~\mathcal{C};~\phi,~\psi)$} \tcp*{contrastive loss} 
%         \textcolor{algohighlight}{$l_{enc}^{clf} \leftarrow \mathcal{L}_{clf}([\mathbf{z^s};\mathbf{z^t}], \mathcal{C}_{i};~\phi,~\psi,~\delta)$}  \tcp*{clf loss}
%         \textcolor{algohighlight}{
%             $\mathcal{L}_{coop} = \lambda_1. l_{enc}^{con}$  + $\lambda_2. l_{enc}^{clf}$
%         } \\ 
%         \textcolor{algohighlight}{$\theta,~\psi \leftarrow Adam(\mathcal{L}_{coop},~\beta_1,~\beta_2,~lr_{ae})$}
%  }
% \caption{Overall training procedure for \systemname{}( + [\textsc{clf}] + [\textsc{contra}]) }
% \label{algo:training-algo}
% \end{algorithm}



\subsection{Adding Constraints via Co-op Training}

While the latent space in \systemname{} learns to match \srcdom{} and \trgdom{} sentences, there is no guarantee on translations maintaining the 
% MinACL: BUG GLOBAL, replace "x" with LaTeX quotes ``x''
``content''. This issue is particularly pronounced in unsupervised attribute transfer due to lack of parallel sentences between \srcdom{} and \trgdom{}.

To alleviate the issue, we propose to learn a structured latent space which embodies notions of our constraints in its embedded latent codes.  This ensure that instances with similar constraints are closer in the latent space. In particular, we propose two types of optimization --- self-supervised and discriminative --- to maintain the constraints better.

\subsubsection{Cooperative Contrastive Learning}

We use contrastive representation learning to regularize the latent space, such that encoders bring two sentences sharing similar constraints closer together (positive pairs), and force dissimilar ones away (negative pairs). For example, sentences of similar lengths (irrespective of their domains) should be closer together.

Among many self-supervised metric losses such as Triplet Loss \cite{tripletloss} and NT-Xent loss \cite{DBLP:conf/icml/ChenK0H20}, we use one that is amenable to multiple positive instances \cite{DBLP:conf/nips/KhoslaTWSTIMLK20}. Given a sentence $s_i \in \mathcal{S}$ in a mini-batch of size $B$, we mine $P$ positive sentences each from \srcdom{} and \trgdom{} that share the same constraints with $s_i$. This contrastive loss is given by:

\small 
\begin{equation}
    \mathcal{L}_{con}(\theta, \psi, \xi) = -\frac{1}{|P|}\log \left( 
        \sum_{j=1}^{P} 
        \frac{
        e^{(\mathbf{z}_i \cdot \mathbf{z}_j)}}{
        \sum_{k=1}^{B\setminus \{i\}} e^{(\mathbf{z}_i \cdot \mathbf{z}_k)}
        }
    \right)
    \label{eq:contra-loss}
\end{equation}
% MinACL: are line references correct/. The reference to line 14 doesn't look correct --- refers to C_i not seen in L14.  Same with L34 (doesn't exist)

\normalsize 
\noindent where $\mathbf{z}$'s are representations obtained from the encoders in \srcdom{}, \trgdom{}  or representations obtained from the last layer of critic $crc_{\xi}$.  $\mathcal{C}_i$ are a set of constraints for a sentence. Recently, \cite{DBLP:conf/nips/KangP20} introduced the cooperative loss in the adversarial setup where contrastive losses are added to both the \textit{critic} and \textit{generator} for GANs. Unlike the normal opposing losses of the generator and the critic, both of them cooperatively reduce the contrastive loss. We follow a similar principle and add the loss to both the encoders and the critic (Lines~18).

\subsubsection{Cooperative Classification}
Contrastive learning might be sub-optimal if we do not mine good quality positive and negative samples \cite{DBLP:conf/nips/Tian0PKSI20}. To address this, we propose another way to regularize the latent space. Similar to ACGAN~\cite{acgan}, we encourage the encoders and the critic to cooperatively reduce a classification loss. 
% Min: how do you predict a constraint?  You mean which constraints are being optimised?  It's not clear to the reader.
We include a classifier $D_{\delta}:\mathcal{Z}\rightarrow\mathbb{R}^{|\mathcal{C}|}$ that predicts the different constraints $\mathcal{C}$ of the sentences
% MinACL: this sentence's two halves don't work well together.  Fix. BUG
and the binary cross entropy loss is reduced.

% MinCR: too big, use smaller font so that the label can fit on the line.

\small 
\begin{align}
\mathcal{L}_{clf}({\theta, \phi, \xi, \delta}) = -\sum_{c=1}^{|\mathcal{C}|} \log{\left(\sigma\left(l_c\right)^{y_c}\left(1 - \sigma\left(l_c\right)\right)^{1-y_c}\right)}
\end{align}

\normalsize
where $|\mathcal{C}|$ is the number of constraints per sentence, $\sigma$ is the sigmoid function and $l_c$ are the logits produced by the classifier for $z_i$. As in contrastive loss, the $z_i$ can be produced by encoders of \srcdom{}, \trgdom{} or from the hidden layers of the critic.

% MinACL: consider putting in a line reference to Alg 1.
The overall training process is highlighted in~\Cref{algo:training-algo} where $\mathcal{L}_{con}$ and $\mathcal{L}_{clf}$ are weighted by $\lambda_1$ and $\lambda_2$. We choose $\lambda_1,~\lambda_2 \in \{0, 1\}$.


% Add all the tips and tricks missing in the ARAE paper but in the implementation 
% Clearly show the simple changes to the algorithm where the contrastive and classification steps are added 
% \paragraph{Training Algorithm:}
% The complete training procedure, as shown in Algorithm~\ref{algo:training-algo}, is similar to standard \arae{} \cite{DBLP:conf/icml/ZhaoKZRL18}. It consists of training autoencoders (Step~1), training the critic (Step~2) and adversarially training the encoders (Step~3).  Step~2a adds the contrastive and cooperative contrastive loss to the critic. This encourages the critic to identify representations that have similar constraints, while the encoders (Step~4) also learn to produce more fine-grained representations that satisfy the constraints as well.


==> Don't change that!/sections/related_work.tex <==
\section{Related Work}

Text attribute transfer has a vast literature \cite{dijin-survey} with deep learning methods becoming popular. The methods are either supervised (requiring parallel data) or unsupervised. Supervised methods re-purpose Sequence to Sequence models used in machine translation to achieve the goals \cite{formality-style-rao}. However, obtaining parallel data is cumbersome and thus unsupervised methods that consider pseudo-parallel data have become popular.  


Disentanglement approaches are the prevalent approach to tackle unsupervised attribute transfer:  \textit{attributes} and \textit{content} are separated in latent dimension. To disentangle the attributes adversarial methods  maximize the loss of a pre-trained attribute classifier  \cite{complementray-aux-classifiers, DBLP:conf/aaai/FuTPZY18, pmlr-v80-zhao18b, john-etal-2019-disentangled}. However, the literature has paid little attention in defining and preserving content. Cycle consistency losses -- imposing that reconstruction from the target style sentence should resemble the source sentence -- is the most prevalent \cite{prabhumoye-etal-2018-style,DBLP:journals/corr/abs-1811-01135, dai-etal-2019-style, huang-etal-2020-cycle, DBLP:conf/ijcai/YiLLS20}. However, this is expensive and non-differentiable, thus requiring reinforcement learning techniques to enforce it. Our work defines the different constraints that should be preserved and adds simple differentiable contrastive learning losses to preserve them.

In recent times, text style transfer models are moving away from disentanglement approaches \cite{multiple-attribute-text-style-transfer}. Recent works that use transformers for style transfer also have adopted this \cite{dai-etal-2019-style, krishna-etal-2020-reformulating}. However, these methods do not explicitly maintain the constraints between the two styles which is the main aim of our work. 


% Inspired by GANs, adversarial methods are prevalent for achieving such disentanglement \cite{pmlr-v80-zhao18b}.  Much of these works transfer a single attribute like, sentiment \cite{pmlr-v80-zhao18b}, expertise \cite{cao-etal-2020-expertise} etc.
% Adversarial methods involve critics that identify attributes. Although applicable to multiple-attribute transfer become infeasible with an increasing number of attributes. Hence, recent works on multiple attribute transfer \cite{multiple-attribute-text-style-transfer} use techniques from unsupervised machine translation  which do not involve critics \cite{artetxe2018unsupervised,lample_unsupervised_mt}. Nonetheless, these works aim to preserve content and ignore other desirable constraints of identity.
% Compared to previous text style transfer works, we aim to maintain these constraints of identity and find that it improves the overall performance. In a similar vein,  \citet{integrating-categorical-semantics-GAN} argue that preserving domain invariant semantic features and identity improves unsupervised image translation.  Also, recent works in CV introduced contrastive learning to GANs \cite{DBLP:conf/nips/KangP20,DBLP:journals/corr/negative_data_augmentation} To the best of our knowledge, we are the first to introduce cooperative losses in the GAN setup for NLP. We discuss other closely related approaches in \Cref{sec:more-related-work}.




% \subsection{Unsupervised Text Generation}
% \begin{itemize}
% \item \cite{huang-etal-2020-cycle} - Cycle consistent adversarial autoencoders
% \item \cite{dai-etal-2019-style} - StyleTransformers 
% \item \cite{DBLP:conf/acl/MadaanSPPNYSBP20} -
% \item \cite{DBLP:conf/emnlp/MaiPMSH20} -
% \item Delete Retrieve Generate
% \item \cite{DBLP:conf/iclr/HeWNB20}
% \item \cite{DBLP:conf/naacl/LiuNW21} using RL.
% \end{itemize}
